On legitimate mining of cryptocurrency in the browser - a feasibility study

Cryptocurrency mining in the browser has the potential to provide a new pay-as-you-go monetisation mechanism for consuming digital media over the Web. However, browser mining has recently received strong criticism due to illegitimate use of mining scripts in several popular websites (a practice called cryptojacking). Here we provide the first feasibility study of browser mining as a legitimate means of monetisation in terms of revenue, user consent and user experience within a specially built website. Our results compare browser mining to display advertisement and indicate browser mining provides a preferable user experience to advertising when the hash rate is user-adjustable. Furthermore, over 60% of participants would select browser mining over advertisement if they were invested in the ecosystem by obtaining half of the mined cryptocurrency. Our estimations show that browser mining currently generates revenue at a rate 46 times less than advertisement, however we would expect that gap to decrease as we observed a significant drop in mining difficulty after our tested cryptocurrency implemented ASIC-resistant mining measures. Overall, based on our results we find browser mining to be a legitimate alternative to display advertisement and conclude by discussing its current limitations and potential applications.

==> sections/relevant_work.tex <==
\section{Related work}
Study by Eskandari et al. \cite{first_look_into_cryptojacking} was among the first to explore browser mining market and estimate mining profitability on 11K parked websites over a three-month period. It also collected a dataset of 33K browser mining websites from censys.io BigQuery to examine CPU usage and found most miners utilised around 25\% of user's CPU which they argued could be considered as fair use. However, there were a few reports of malicious use which utilised 100\% of CPU. The authors also provided the first framework for evaluating the ethical aspects of browser mining suggesting current methods of informed consent collection could be inadequate. Their conclusion was that the ethics of browser mining are not yet fully understood and require further discussion. Papadopoulos et al. \cite{truth_about_cryptomining} extended evaluation of browser mining feasibility by comparing profitability from online ads and browser mining on a combined dataset of 200K ad and mining enabled websites and found the former to be 5.5x more profitable, however their study also indicated that browser mining could be more profitable if the browsing session exceeds 5.3 minutes. In addition, they compared CPU utilisation and estimated user costs on both monetisation options. Their findings suggest the median CPU usage when mining was 59x higher. Considering the results, Papadopoulos et al. proposed a new model of monetisation which would allow users to choose between ads and browser mining, whilst informing them about implicit costs from both options.
